SteelCore: An Extensible Concurrent Separation Logic for Effectful Dependently Typed Programs

Much recent research has been devoted to modeling effects within type theory. Building on this work, we observe that effectful type theories can provide a foundation on which to build semantics for more complex programming constructs and program logics, extending the reasoning principles that apply within the host effectful type theory itself. Concretely, our main contribution is a semantics for concurrent separation logic (CSL) within the F* proof assistant in a manner that enables dependently typed, effectful F* programs to make use of concurrency and to be specified and verified using a full-featured, extensible CSL. In contrast to prior approaches, we directly derive the partial-correctness Hoare rules for CSL from the denotation of computations in the effectful semantics of non-deterministically interleaved atomic actions. Demonstrating the flexibility of our semantics, we build generic, verified libraries that support various concurrency constructs, ranging from dynamically allocated, storable spin locks, to protocol-indexed channels. We conclude that our effectful semantics provides a simple yet expressive basis on which to layer domain-specific languages and logics for verified, concurrent programming.

==> lstfstar.tex <==
\newcommand\function{\sffamily\maybecolor{dkblue}function}

\makeatletter
\lstdefinelanguage{fstar}{%
  basicstyle=\small,
  morekeywords=[1]{type,and,val,fun,let,in,ref,uref,mref,try,if,then,else,match,with,open,as,module,rec,begin,end,assume,private,when,forall,assert,by_tactic,logic,array,pattern,effect,requires,ensures,decreases,modifies, abstract,total, reifiable, reflectable, new_effect, effect_actions, noeq, sub_effect, by, synth,splice},
  morekeywords=[2]{WP, Post, Pre, Pure , PURE, DIV, Dv, STATE, EXN, ALL, TotST, M, GHOST, Ghost, GTot, Lemma, Tot, Div, DIV, Memo, READER, STATE_m, Effect, STEXN, RANDOM, ST, St, MST, S_MST, MSTExn, TAC, Tac, TacH, Type},
  morekeywords=[3]{},
  morekeywords=[4]{},
  morestring=[b]",
  sensitive=true,%
  numbersep=4pt,
%  numbers=left,
  columns=[l]fullflexible,
  texcl=true,
  mathescape=true,
%  xleftmargin=10pt,
  identifierstyle={\sffamily},
  keywordstyle=[1]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[2]{\sffamily\maybecolor{dkblue}},
  keywordstyle=[3]{\maybecolor{dkred}},
  keywordstyle=[4]{\rmfamily\itshape},
% Here is the range marker stuff
  rangeprefix=(*---\ ,
  includerangemarker=false,
  stringstyle=\ttfamily,
  %lineskip=-2pt,
  showspaces=false,
  morecomment=[n]{(*}{*)},
  commentstyle={\itshape\maybecolor{dkred}},
  literate={->}{$\rightarrow\,$}{1}
           {True}{$\top$}{1}
           {False}{$\bot$}{1}
           {exists}{$\exists$}{1}
           {forall}{$\forall$}{1}
           {fun}{$\lambda$}{1}
           {~}{$\neg$}{1}           
           {~>}{$\leadsto$}{1}
           {`}{\`{}}{1}
           {'a}{$\alpha$}{1}
           {'b}{$\beta$}{1}
           {'c}{$\gamma$}{1}
           {`star`}{$\ast\,$}{1}           
           {-*}{$\mbox{\endash}\ast\,$}{1}                      
           {Gamma}{$\Gamma\,$}{1}
           {theta}{$\theta\,$}{1}
           {_0}{$_0$}{1}
           {_1}{$_1$}{1}
           {_2}{$_2$}{1}
           {_3}{$_3$}{1}
           {_4}{$_4$}{1}
           {/\\}{$\wedge\;$}{1}
           {\\/}{$\vee\;$}{1}
           {>=}{$\geq\ $}{2}
           {<=}{$\leq\ $}{2}
           {<==>}{$\Longleftrightarrow \ $}{3}
           {==>}{$\Longrightarrow \ $}{3}
           {|->}{$\mapsto \ $}{3}
           {<>}{$\neq$}{1}
           {--}{-}{1}   % Added due to         - not displaying properly.  Weird. ... but may make arrows look bad  {...}{$\ldots$}{3}
           {<<}{$\prec\ $}{1}
           ,
  breaklines=false}
\makeatother

